Learning from Irregularly-Sampled Time Series: A Missing Data Perspective

Irregularly-sampled time series occur in many domains including healthcare. They can be challenging to model because they do not naturally yield a fixed-dimensional representation as required by many standard machine learning models. In this paper, we consider irregular sampling from the perspective of missing data. We model observed irregularly-sampled time series data as a sequence of index-value pairs sampled from a continuous but unobserved function. We introduce an encoder-decoder framework for learning from such generic indexed sequences. We propose learning methods for this framework based on variational autoencoders and generative adversarial networks. For continuous irregularly-sampled time series, we introduce continuous convolutional layers that can efficiently interface with existing neural network architectures. Experiments show that our models are able to achieve competitive or better classification results on irregularly-sampled multivariate time series compared to recent RNN models while offering significantly faster training times.

==> alternatives.tex <==
\section{Alternative Models}

In addition to P-VAE and P-BiGAN introduced in Section~\ref{sec:framework},
here we present alternative models and their variations
for training the encoder-decoder framework.
In P-BiGAN, we include the autoencoding loss in the objective
as in \eqref{eq:p-bigan-ae},
In fact, this somewhat serves the same purpose of discriminating
the generated incomplete data $(\xx,\tt)$ from the real ones sampled
from the training data.
Therefore, we can simplify P-BiGAN by discriminating only the
encoding latent codes and the sampled ones.
The resulting model is then similar to the adversarial autoencoder
\citep{makhzani2015adversarial,tolstikhin2018wasserstein},
which we call P-AAE.
Specifically, P-AAE is trained with
\begin{align*}
  \min_{\theta,\phi}\max_D\
  &\E_{\zz\sim p_z(\zz)}\left[\log D(\zz)\right] \\
  &+ \E_{(\xx,\tt)\sim p_\D}\left[\E_{\zz\sim p_\phi(\zz|\xx,\tt)}
  \left[\log(1 - D(\zz))\right]\right] \\
  &+ \lambda \E_{\zz\sim q_\phi(\zz|\xx,\tt)}\Bigg[
  \sum_{i=1}^{|\tt|} \ell\big(x_i, g_\theta(\zz,t_i)\big)\Bigg].
\end{align*}
However, in the image modeling experiments in Section~\ref{sec:impute fid},
we found that P-AAE usually fails to learn a reasonable generative model
under the same architecture used by P-BiGAN.
Further investigation of this model is left for future work.

Alternatively, we can also split the discriminator that
originally operates on the joint of
the incomplete data $(\xx,\tt)$ and the latent code $\zz$
into two separate parts,
and use the autoencoder to enforce the invertibility relationship
between the encoder and the decoder to achieve the consistency between
$(\xx,\tt)$ and $\zz$.
Specifically, the resulting model is trained using
\begin{align*}
  \min_{\theta,\phi}\max_{D_x, D_z}\
  &\lambda \E_{\zz\sim q_\phi(\zz|\xx,\tt)}\Bigg[
  \sum_{i=1}^{|\tt|} \ell\big(x_i, g_\theta(\zz,t_i)\big)\Bigg] \\
  &+ \alpha\E_{(\xx,\tt)\sim p_\D}\left[\log D_x(\xx,\tt)\right] \\
  &+ \alpha\E_{\zz\sim p_z(\zz)}\E_{(\xx,\tt)\sim p_\D}\left[
    \log (1 - D_x(g_\theta(\zz,\tt),\tt))
  \right] \\
  &+ \E_{\zz\sim p_z(\zz)}\left[\log D_z(\zz)\right] \\
  &+ \E_{(\xx,\tt)\sim p_\D}\left[\E_{\zz\sim p_\phi(\zz|\xx,\tt)}
  \left[\log(1 - D_z(\zz))\right]\right].
\end{align*}
The additional hyperparameter $\alpha$ controls the strength
of discriminating the incomplete data,
which makes P-AAE a special case when $\alpha=0$.

By splitting the discriminator into two parts,
we can use different loss functions for the two separate GANs.
% such as using MMD-GAN \citep{li2017mmd} for $\zz$.
In fact, since the Gaussian prior we use for $p_z$
has a relatively simple structure,
we can even directly use MMD with an RBF-kernel without learning
a discriminator for $\zz$ to speed up training,
which also makes the optimization more stable.

We also note that if we only need to learn the generative model $g_\theta$,
it is sufficient to train $g_\theta$ alone with
the following optimization problem
without the presence of the encoder $q_\phi$,
which is essentially a MisGAN without the imputer
and the generator/discriminator for masks:
\begin{align*}
  \min_{\theta}\max_{D_x, D_z}\
  & \E_{(\xx,\tt)\sim p_\D}\left[\log D_x(\xx,\tt)\right] \\
  &+ \E_{\zz\sim p_z(\zz)}\E_{(\xx,\tt)\sim p_\D}\left[
    \log (1 - D_x(g_\theta(\zz,\tt),\tt))
  \right].
\end{align*}



==> errata.tex <==
\section{Errata}

\textbf{Definition~\ref{def:masking}:}
The definition of each entry of $\vv=m(\xx,\tt)$ 
in the original submission was 
\[
v_t = \sum_{i\in\I} x_i\1\{t_i=t\}. 
\]
It should be
\[
v_t = \sum_{i=1}^{|\tt|} x_i\1\{t_i=t\}.
\]

